Integration of Imitation Learning using GAIL and Reinforcement Learning using Task-achievement Rewards via Probabilistic Graphical Model

Integration of reinforcement learning and imitation learning is an important problem that has been studied for a long time in the field of intelligent robotics. Reinforcement learning optimizes policies to maximize the cumulative reward, whereas imitation learning attempts to extract general knowledge about the trajectories demonstrated by experts, i.e., demonstrators. Because each of them has their own drawbacks, methods combining them and compensating for each set of drawbacks have been explored thus far. However, many of the methods are heuristic and do not have a solid theoretical basis. In this paper, we present a new theory for integrating reinforcement and imitation learning by extending the probabilistic generative model framework for reinforcement learning, {\it plan by inference}. We develop a new probabilistic graphical model for reinforcement learning with multiple types of rewards and a probabilistic graphical model for Markov decision processes with multiple optimality emissions (pMDP-MO). Furthermore, we demonstrate that the integrated learning method of reinforcement learning and imitation learning can be formulated as a probabilistic inference of policies on pMDP-MO by considering the output of the discriminator in generative adversarial imitation learning as an additional optimal emission observation. We adapt the generative adversarial imitation learning and task-achievement reward to our proposed framework, achieving significantly better performance than agents trained with reinforcement learning or imitation learning alone. Experiments demonstrate that our framework successfully integrates imitation and reinforcement learning even when the number of demonstrators is only a few.

==> figures/graphical1.tex <==

%\begin{wrapfigure}{r}{60mm}
%    \centering
\begin{figure}{}
    \begin{center}
        \tikzstyle{obs}=[shape=circle,draw=black!50,fill=gray!20]
        \tikzstyle{state}=[shape=circle,draw=black!50,fill=white!20]
        \tikzstyle{action}=[shape=circle,draw=black!50,fill=white!20]
        \tikzstyle{lightedge}=[<-,thick]
        \tikzstyle{bendedge}=[<-,bend left=38]
        \tikzstyle{bendedge2}=[<-,bend left=30]
        \newcommand{\wrat}{1.4}
        \begin{tabular}{c}
            \begin{minipage}{0.5\linewidth}
                \centering
                \begin{tikzpicture}[]
                    \node[action] (a1) at (0*\wrat,2) {$\ba_1$};
                    \node[action] (a2) at (1*\wrat,2) {$\ba_2$};
                    \node[action] (a3) at (2*\wrat,2) {$\ba_3$};
                    \node[action] (a4) at (3*\wrat,2) {$\ba_4$};
                    
                    \node[state] (s1) at (0*\wrat,1) {$\bs_1$};
                    \node[state] (s2) at (1*\wrat,1) {$\bs_2$}
                        edge [lightedge] (s1)
                        edge [lightedge] (a1);
                    \node[state] (s3) at (2*\wrat,1) {$\bs_3$}
                        edge [lightedge] (s2)
                        edge [lightedge] (a2);
                    \node[state] (s4) at (3*\wrat,1) {$\bs_4$}
                        edge [lightedge] (s3)
                        edge [lightedge] (a3);
                \end{tikzpicture}
            \end{minipage}
            \begin{minipage}{0.5\linewidth}
                \centering
                \begin{tikzpicture}[]
                    \node[action] (a1) at (0*\wrat,2) {$\ba_1$};
                    \node[action] (a2) at (1*\wrat,2) {$\ba_2$};
                    \node[action] (a3) at (2*\wrat,2) {$\ba_3$};
                    \node[action] (a4) at (3*\wrat,2) {$\ba_4$};
                    
                    \node[state] (s1) at (0*\wrat,1) {$\bs_1$};
                    \node[state] (s2) at (1*\wrat,1) {$\bs_2$}
                        edge [lightedge] (s1)
                        edge [lightedge] (a1);
                    \node[state] (s3) at (2*\wrat,1) {$\bs_3$}
                        edge [lightedge] (s2)
                        edge [lightedge] (a2);
                    \node[state] (s4) at (3*\wrat,1) {$\bs_4$}
                        edge [lightedge] (s3)
                        edge [lightedge] (a3);
                    
                    \node[obs] (o1) at (0*\wrat,3.25) {$\op_1$}
                        edge [bendedge] (s1)
                        edge [lightedge] (a1);
                    \node[obs] (o2) at (1*\wrat,3.25) {$\op_2$}
                        edge [bendedge] (s2)
                        edge [lightedge] (a2);
                    \node[obs] (o3) at (2*\wrat,3.25) {$\op_3$}
                        edge [bendedge] (s3)
                        edge [lightedge] (a3);
                    \node[obs] (o4) at (3*\wrat,3.25) {$\op_4$}
                        edge [bendedge] (s4)
                        edge [lightedge] (a4);
                \end{tikzpicture}
            \end{minipage}
        \end{tabular}
      \caption{Left: A graphical model of MDP having states and actions as stochastic variables. Right: A graphical model for reinforcement learning as probabilistic inference. The agent observes single optimality $\op_t$ every timestep and infers the most probable action on the conditioning the optimality variables being true. In this paper, we call the graphical model a probabilistic graphical model fro Markov decision process (pMDP).} 
      \label{fig:sub1}
  \end{center}
\end{figure}
%\end{wrapfigure}

==> figures/graphical2.tex <==
\begin{figure}[]
    \centering
    \tikzstyle{obs}=[shape=circle,draw=black!50,fill=gray!20]
    \tikzstyle{state}=[shape=circle,draw=black!50,fill=white!20]
    \tikzstyle{action}=[shape=circle,draw=black!50,fill=white!20]
    \tikzstyle{lightedge}=[<-,thick]
    \tikzstyle{bendedge}=[<-,bend left=38]
    \tikzstyle{bendedge2}=[<-,bend left=30]
    \newcommand{\wrat}{1.4}
    \begin{tikzpicture}[]
        \node[action] (a1) at (0*\wrat,2) {$\ba_1$};
        \node[action] (a2) at (1*\wrat,2) {$\ba_2$};
        \node[action] (a3) at (2*\wrat,2) {$\ba_3$};
        \node[action] (a4) at (3*\wrat,2) {$\ba_4$};
        
        \node[state] (s1) at (0*\wrat,1) {$\bs_1$};
        \node[state] (s2) at (1*\wrat,1) {$\bs_2$}
            edge [lightedge] (s1)
            edge [lightedge] (a1);
        \node[state] (s3) at (2*\wrat,1) {$\bs_3$}
            edge [lightedge] (s2)
            edge [lightedge] (a2);
        \node[state] (s4) at (3*\wrat,1) {$\bs_4$}
            edge [lightedge] (s3)
            edge [lightedge] (a3);
        
        \node[obs] (og1) at (0*\wrat,3.25) {$\op_1^1$}
            edge [bendedge] (s1)
            edge [lightedge] (a1);
        \node[obs] (og2) at (1*\wrat,3.25) {$\op_2^1$}
            edge [bendedge] (s2)
            edge [lightedge] (a2);
        \node[obs] (og3) at (2*\wrat,3.25) {$\op_3^1$}
            edge [bendedge] (s3)
            edge [lightedge] (a3);
        \node[obs] (og4) at (3*\wrat,3.25) {$\op_4^1$}
            edge [bendedge] (s4)
            edge [lightedge] (a4);
        
        
        \node at (0*\wrat,4.2) {\vdots};
        \node at (1*\wrat,4.2) {\vdots};
        \node at (2*\wrat,4.2) {\vdots};
        \node at (3*\wrat,4.2) {\vdots};
        
        \node[obs] (od1) at (0*\wrat,5.0) {$\op_1^N$}
            edge [bendedge] (s1)
            edge [bendedge] (a1);
        \node[obs] (od2) at (1*\wrat,5.0) {$\op_2^N$}
            edge [bendedge] (s2)
            edge [bendedge] (a2);
        \node[obs] (od3) at (2*\wrat,5.0) {$\op_3^N$}
            edge [bendedge] (s3)
            edge [bendedge] (a3);
        \node[obs] (od4) at (3*\wrat,5.0) {$\op_4^N$}
            edge [bendedge] (s4)
            edge [bendedge] (a4);


    \end{tikzpicture}
    
    
      \caption{A graphical model framework for reinforcement learning as probabilistic inference with multiple optimal emissions. In this framework, agent observes multiple optimalities $\op_t^1, ..., \op_t^N$ and inferences the optimal behavior.}
      \label{fig:sub2}
\end{figure}

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

